Towards Trustworthy Embodied Intelligence: A Systems Framework and Graded Trustworthiness Levels

Embodied intelligence integrates learned perception and decision making with real-time computation, control, and physical interaction. Because failures can cause immediate physical or operational harm, task completion alone does not establish trustworthiness. We define trustworthy embodied intelligence as the sustained capacity to execute specified tasks reliably under environmental and system variation while maintaining risk within acceptable bounds. We term this objective sustained safe success. Its supporting mechanisms are organized into four interdependent layers. The model layer generates task-competent action proposals with calibrated uncertainty and explicit safety preferences. The system layer realizes authorized actions dependably through integrated sensing, computation, control, hardware safeguards, fault containment, and fallback. The evidence layer substantiates bounded claims through evaluation, verification, validation, traceability, and structured assurance arguments. The deployment layer maintains claim validity through runtime monitoring, authority management, intervention, incident response, and controlled updates. Because assumptions and failures propagate across these layers, neither model capability, isolated safeguards, nor benchmark performance alone can establish end-to-end trustworthiness. Drawing on embodied AI, robotics, control, dependable computing, distributed systems, and autonomous driving, we further propose a non-normative hierarchy of trustworthiness levels. This hierarchy grades the strength of bounded deployment claims across task capability, safety, system assurance, operational governance, and supporting evidence, providing a basis for bounded deployment, comparative evaluation, research prioritization, and future standardization.

==> sections/_bac_2_foundations.tex <==
\section{Foundations of Trustworthy Physical Intelligence}
\label{sec:foundations}

Trustworthy physical intelligence is an integration problem built on mature engineering foundations. Learned perception, reasoning, planning, and control provide the capabilities required to complete physical tasks, while dependable computing, networked systems, feedback control, and physical safety mechanisms determine whether those capabilities can be exercised reliably and within acceptable risk. Dependable computing explains how faults propagate into externally visible failures and how isolation, redundancy, and recovery contain them. Operating systems motivate privilege boundaries between complex intelligence and physical authority. Computer networks and distributed systems expose partial failure, untrusted communication, and timing uncertainty. Robotics and control provide the foundations for feedback, stability, observability, controllability, contact regulation, and energy limitation. These foundations are not merely analogies: they provide reusable design principles while revealing where physical embodiment makes capability and safety difficult to sustain jointly.

\subsection{Dependable Computer Systems: Faults, Isolation, and Privilege}
\label{subsec:computer_systems}

A classical dependability chain distinguishes a \emph{fault}, an \emph{error}, and a \emph{failure}~\citep{avizienis2004dependability}. A fault is a defect or abnormal condition, such as sensor drift, a bit flip, a flawed model update, incorrect calibration, or a compromised software dependency. The fault creates an erroneous internal state only when activated, and a system failure occurs when that error crosses an interface and prevents the delivered service from satisfying its specification. This distinction is important for embodied intelligence because an error in perception, reasoning, or planning need not become a physical failure if it is detected, rejected, masked, or corrected before reaching actuation.

Dependable systems employ four complementary strategies. Fault prevention reduces defects through disciplined development, verification, configuration control, and secure supply chains. Fault removal identifies and corrects defects through testing and analysis. Fault tolerance preserves acceptable service despite faults through redundancy, reconfiguration, voting, and graceful degradation~\citep{gao2015faultsurvey}. Fault forecasting estimates the likelihood and consequence of future failures to guide design and maintenance. Embodied systems require all four: learning cannot replace engineering discipline, and redundant components cannot compensate for a shared erroneous model, calibration process, timing source, or power dependency.

Operating systems provide a second foundation. User applications are separated from a privileged kernel because they are complex, frequently updated, and not assumed to be correct. Access to memory, devices, networks, and other protected resources is mediated through controlled interfaces. The analogous design for embodied AI treats a foundation model or task planner as a capable but non-privileged component. It may interpret goals and propose skills, but it should not directly issue unrestricted actuator commands. Robot capabilities can instead be exposed as typed operations with declared preconditions, permissions, resource and risk bounds, postconditions, timeouts, monitor signals, and recovery procedures.

This design motivates a small trusted computing base for physical action. A reference monitor should be tamper-resistant, always invoked, and sufficiently simple to analyze~\citep{saltzer1975protection}. In robotics, this function may be distributed across a capability gate, safety controller, watchdog, hardware interlock, and human stop mechanism. Least privilege restricts an agent to the capabilities required for its current task. Isolation prevents failures in perception, planning, logging, or external tools from corrupting safety-related control. Watchdogs detect stalled processes and missed deadlines, while audit logs record which principal proposed, authorized, modified, and executed an action.

The analogy has important limits. Physical state generally cannot be restored from a memory snapshot: a dropped object, collision, spill, or injury may be irreversible. Recovery is therefore closer to a compensating transaction than a digital rollback. The system must first reach a safe physical condition, assess the resulting state, and then either restore valid task preconditions or terminate. Likewise, simply stopping all computation may be unsafe for a balancing humanoid, airborne drone, moving vehicle, or robot supporting a load. Depending on the physical context, the system must choose between fail-safe stopping and fail-operational degradation while preserving enough capability to reach a minimum-risk state.

\subsection{Computer Networks and Distributed Systems: Time, Trust, and Partial Failure}
\label{subsec:computer_networks}

Modern robots are distributed systems. Sensors, embedded controllers, accelerators, edge computers, cloud models, operator stations, digital twins, and peer robots communicate over buses and networks with different latency, bandwidth, reliability, and trust assumptions. Communication behavior therefore becomes part of the physical system dynamics. Delay and jitter can destabilize feedback; packet loss can create stale state; message reordering can violate command-sequence assumptions; clock drift can corrupt sensor fusion and incident reconstruction; and network partitions can leave components with inconsistent views of the world.

A network-inspired separation among control, operational data, and governance responsibilities is useful. A relatively slow semantic layer selects goals, tasks, routes, and capabilities. High-rate sensing and actuation carry the data that directly drives the physical process. Governance mechanisms define identities, permissions, constraints, escalation policies, and audit requirements. Mixing these responsibilities creates fragile architectures: a cloud planner should not occupy a sub-millisecond reflex path, a high-rate servo should not determine whether a natural-language request is authorized, and the component proposing an action should not be the sole judge of whether that action may execute.

Distributed systems exhibit partial rather than total failure. A cloud model may become unavailable while local control remains healthy; one sensor may be compromised while another remains valid; a robot may lose coordination messages while continuing to move; and an operator interface may display stale information even though the robot is functioning. The system must define behavior for each degraded condition rather than assume a binary distinction between normal operation and complete shutdown. Heartbeats, sequence numbers, freshness bounds, redundant paths, local caches, restricted operating modes, and explicit partition behavior support both continued task execution and risk containment.

Security mechanisms are part of the same physical assurance boundary. Authentication establishes which human, service, robot, or model is requesting an action. Authorization limits what that identity may do. Integrity and anti-replay protection prevent commands from being modified or repeated, while segmentation limits lateral movement after compromise. Continuous verification avoids granting permanent trust because a component passed one initial check~\citep{rose2020zerotrust}. In multi-robot systems, Byzantine or inconsistent peers require robust coordination, shared-resource arbitration, and local collision avoidance that do not depend on universal cooperation~\citep{lamport1982byzantine}.

Timing deserves particular attention. A measurement without a trustworthy timestamp may be worse than no measurement because it silently violates the estimator's assumptions, and a numerically valid command may become unsafe when delivered too late~\citep{sha1990priority}. End-to-end latency includes sensing, transport, scheduling, model inference, policy generation, command transmission, actuator response, and physical dynamics. Optimizing model inference alone therefore misses the quantity that determines whether useful and safe action remains possible. Trustworthiness claims should specify deadline budgets, tail or worst-case latency, synchronization assumptions, and the behavior triggered by deadline violations.

\subsection{Robotics and Control: Feedback, Safety, and Multiple Time Scales}
\label{subsec:robotics_foundations}

An embodied agent operates through feedback. In a simplified discrete-time model,
\begin{equation}
    x_{t+1}=f(x_t,u_t,w_t), \qquad y_t=h(x_t,v_t),
\end{equation}
where $x_t$ is the physical state, $u_t$ is the control action, $w_t$ represents disturbances and unmodeled dynamics, $y_t$ is the observation, and $v_t$ represents sensing error. A learned model acts on an estimate $\hat{x}_t$ rather than the complete physical state. Its ability to complete a task safely therefore depends on estimation quality, sensitivity to model error, available control authority, and the response when uncertainty or deviation becomes excessive.

Several system properties must be distinguished. Stability asks whether trajectories remain bounded or converge. Performance concerns how accurately, efficiently, and promptly the task is completed. Safety asks whether the system avoids hazard states or remains within an acceptable set~\citep{isoiec2014guide51}. Reliability concerns whether required service continues over time. Observability asks whether relevant internal states can be inferred from available measurements, and controllability asks whether available inputs can drive the system toward desired or safe states. These properties support one another but are not interchangeable: a stable robot may exert unsafe force, a reliable controller may repeatedly execute an unsafe goal, and a detected hazard may remain unavoidable when control authority or stopping distance is insufficient.

Control-theoretic safety often defines a safe set $\mathcal{S}$ and seeks to maintain forward invariance: if $x_0\in\mathcal{S}$, then $x_t\in\mathcal{S}$ for all relevant times. Barrier functions~\citep{ames2019cbf}, reachability methods~\citep{bansal2017reachability}, robust model predictive control~\citep{mayne2000constrained}, and invariant-set methods can enforce such conditions when the dynamics, uncertainty bounds, and constraints are credible. These methods provide strong but local evidence. They cannot interpret an ambiguous instruction, determine whether a task is authorized, or repair an incomplete semantic specification. Their applicability also weakens when contact modes, deformable materials, human behavior, and learned high-dimensional policies invalidate simplified models.

Embodied systems are naturally multi-rate. Semantic reasoning and long-horizon planning may operate at fractions of a hertz to a few hertz, skill or VLA policies at an intermediate rate, and torque control, impedance regulation, balance, collision detection~\citep{haddadin2017collisions}, and hardware interlocks at much higher rates~\citep{hogan1984impedance}. This hierarchy is sometimes described as a slow brain, fast brain, and spinal reflex, but its engineering significance lies in the separation of responsibilities. High-level reasoning supplies context and task adaptation; intermediate policies coordinate useful behavior; and local loops preserve timing, stability, force limits, and immediate hazard response. No high-level model, however capable, can compensate for a missed deadline during a high-energy contact event.

Physical human--robot interaction adds energy and biomechanics to the analysis. Risk depends on speed, effective mass, contact area, body region, stiffness, force, pressure, power, duration, and whether a person can recoil or is clamped~\citep{isots15066}. The proper object of analysis is therefore the configured application rather than the robot model alone. A lightweight compliant arm may become hazardous when carrying a sharp or heavy tool, while reliable context perception and effective-mass estimation may allow less conservative motion than fixed worst-case limits. Useful capability and physical safety must consequently be co-designed rather than optimized independently~\citep{zanella2026phri}.

\subsection{Trustworthy Autonomous Driving as an Engineering Analogue}
\label{subsec:autonomous_driving_transfer}

Autonomous driving provides a productive engineering comparison because it combines learned perception and prediction, networked computation, real-time control, human interaction, physical risk, and large-scale deployment. Several mechanisms transfer to broader embodied systems. An operational design domain (ODD) specifies where, when, and under which road, weather, speed, traffic, map, and infrastructure conditions a function is intended to operate~\citep{iso21448}. Scenario-based validation targets meaningful combinations of actors and events rather than relying only on aggregate distance~\citep{riedmaier2020scenario}. Virtual proving grounds make hazardous and rare cases repeatable. Independent monitors and fallback behavior provide minimum-risk responses when assumptions fail, while event data and fleet monitoring support incident analysis and controlled updates.

For embodied intelligence, an equivalent operating domain must include the robot body, sensors, tools, payload, workspace, object classes, contact modes, human proximity, network conditions, task language, and authority structure. A household robot authorized to carry soft objects in one room is not thereby qualified to manipulate knives near children. Similarly, validation on one gripper, camera, payload, or controller does not automatically transfer after an embodiment or configuration change. Deployment claims must therefore be task-, embodiment-, and contact-specific rather than stated only in broad terms such as ``indoors'' or ``in factories.''


Important differences limit direct transfer. Driving is highly complex
but constrained by road geometry, vehicle dynamics, and a comparatively
stable rule structure. General-purpose robots use diverse tools,
intentionally make contact, manipulate materials with uncertain friction
and compliance, and interpret open-ended language. Contact that is
normally undesirable in driving may be essential to manipulation. A
minimum-risk stop is often well defined for a vehicle but may itself be
dangerous for a robot carrying a person, supporting a load, maintaining
balance, or holding a fragile object. Trustworthy embodied intelligence
should therefore adapt driving practices rather than reproduce them
unchanged.

Despite these differences, the engineering domains discussed above provide complementary foundations for trustworthy physical intelligence. Dependable computing contributes fault containment and recovery; operating systems contribute privilege separation and isolation; distributed systems contribute timing awareness and partial-failure handling; robotics and control contribute feedback-based physical safety; and autonomous driving contributes bounded deployment and scenario-based assurance. Table~\ref{tab:foundation_matrix} provides a compact comparison of these contributions.

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.25}
\caption{Complementary engineering foundations for trustworthy physical
intelligence. A checkmark denotes a primary contribution of the
corresponding field rather than complete coverage of the assurance
capability.}
\label{tab:foundation_matrix}

\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\textbf{Engineering foundation}
&
\textbf{Faults}
&
\textbf{Privilege}
&
\textbf{Partial failure}
&
\textbf{Timing}
&
\textbf{Monitoring}
&
\textbf{Degradation}
&
\textbf{Physical safety}
&
\textbf{Deployment evidence}
\\
\midrule

Dependable computing
&
$\checkmark$
&
&
&
&
$\checkmark$
&
$\checkmark$
&
&
\\

Operating systems
&
&
$\checkmark$
&
&
&
$\checkmark$
&
&
&
\\

Networks and distributed systems
&
&
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
&
\\

Robotics and control
&
&
&
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
\\

Autonomous driving
&
&
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
\\

\bottomrule
\end{tabular}%
}
\end{table}

The matrix highlights that no single engineering foundation covers the complete assurance problem. Their mechanisms address different parts of the perception--decision--action loop and must therefore be integrated across system layers. Moreover, the checkmarks represent transferable engineering capabilities rather than guarantees that the corresponding problem has been fully solved for embodied intelligence. Physical embodiment introduces open-ended semantic instructions, state-dependent and potentially irreversible consequences, and interactions among components whose local guarantees may not compose. These remaining difficulties can be summarized as three structural gaps.


\subsection{Three Structural Gaps}
\label{subsec:semantic_physical_gaps}



The first structural gap is the \emph{semantic--physical gap}. Language and symbolic plans express intent compactly but omit geometry, force, friction, timing, material properties, and intermediate feedback. A plan may be linguistically coherent and aligned with the user's words while remaining physically infeasible or hazardous. Modifiers such as ``quickly,'' ``carefully,'' or ``clear the table'' do not uniquely determine control parameters or risk limits. Grounding must therefore translate semantic objectives and constraints into explicit physical interfaces while preserving their rationale and uncertainty~\citep{ma2026breaks}.

The second is the \emph{action--consequence gap}. Physical outcomes are state-dependent and nonlinear. The same end-effector displacement may be effective and safe when an object is light and centered, but ineffective or hazardous when it is heavy, near an edge, partially obstructed, or already slipping~\citep{kojima2025physicalrisk}. Small pose errors can change contact modes, actuator saturation can convert a feasible trajectory into tracking failure, and a delayed command can become unsafe even when its numeric value is correct. Static action whitelists and one-time plan checks cannot capture this dependence on evolving physical state.

The third is \emph{cross-layer non-compositionality}. A perception module may satisfy its accuracy target, a planner may generate a collision-free path in its internal model, and a controller may track that path stably, yet the integrated system may still fail the task or violate safety constraints. Objectives differ across layers, uncertainty is compressed or discarded at interfaces, constraints use incompatible representations, and components operate at different rates. Local guarantees also fail to compose across time: individually acceptable actions may accumulate risk, invalidate later preconditions, degrade task recoverability, or lead to an unsafe success. End-to-end trustworthiness therefore requires shared invariants, explicit cross-layer contracts, continuous feedback, and evidence directed at the integrated perception--decision--action loop~\citep{kim2026longhorizon,ma2026breaks}.

==> sections/_bac_5_hardware_trustworthiness.tex <==
\section{Hardware Trustworthiness}
\label{sec:hardware}

The physical-execution plane determines whether an authorized action can be observed, computed, communicated, controlled, and realized within physical limits. It includes sensors and tactile interfaces, embedded and edge processors, buses and networks, power and thermal systems, actuators, brakes, mechanical structures, tools, and safety-related control hardware. Hardware is therefore not merely a substrate for intelligent software. It determines which task-relevant states are observable, which actions are feasible, which deadlines can be met, how accurately intended behavior can be executed, how much energy can be released, and which degraded states remain controllable.

Hardware trustworthiness must be evaluated at the level of the configured system, task, and environment rather than inferred from individual component quality. A reliable sensor may be poorly positioned; redundant channels may share calibration, timing, compute, or power dependencies; a compliant arm may become hazardous when equipped with a heavy or sharp tool; and a high-performance processor may violate control deadlines after thermal throttling. The relevant question is whether the physical system can sustain useful task performance while preserving sufficient observability, control authority, and risk margins under expected variation and faults. Figure~\ref{fig:hardware_trust_chain} summarizes this closed loop from sensing through computation and actuation to the physical environment, together with the cross-cutting mechanisms that support degradation and transition to a minimum-risk state.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{assets/figures/5_hardware_trust_chain_en.pdf}
  \caption{Hardware trust chain for embodied systems. Solid black arrows denote
  data and command flow across the physical-execution loop; the dashed red
  arrow denotes a fast local protection path from tactile sensing to actuation;
  and the blue arrow denotes feedback through the physical environment.
  Cross-cutting sensing, diagnosis, control, and mechanical safeguards support
  continued operation, controlled degradation, or transition to a minimum-risk
  state.}
  \label{fig:hardware_trust_chain}
\end{figure*}

\subsection{Sensors and Tactile Perception}
\label{subsec:sensors_tactile}

Sensors determine which physical states, hazards, and capability limits are observable. Their faults include bias, drift, saturation, dropout, noise, misalignment, contamination, temperature sensitivity, aging, and electromagnetic or acoustic interference. Digital interfaces add packet loss, stale buffers, timestamp errors, and corrupted configuration. Abrupt faults may produce clear discontinuities, whereas gradual faults can remain plausible while degrading task accuracy and eroding safety margins.

Redundancy is useful only when shared dependencies are understood. Identical cameras may fail under the same glare, darkness, contamination, or adversarial pattern, and otherwise diverse sensors may still depend on a common clock, processor, power rail, coordinate frame, or calibration pipeline. Multimodal sensing should therefore record health, uncertainty, freshness, calibration status, and dependency structure rather than treat channels as interchangeable votes~\citep{avizienis2004dependability}. When modalities disagree, fusion mechanisms should account for risk, sensor condition, and the physical quantity being measured instead of resolving conflict through confidence scores alone.

Sensor placement and coverage are as important as nominal accuracy. Blind regions, self-occlusion, limited field of view, vibration, cable motion, tool obstruction, and changes in robot configuration alter what can be observed during execution. Coverage analysis should consider whether a person, body part, obstacle, or moving object can enter an unobserved region before the system can detect the change and respond. It should therefore include robot motion, tool configuration, stopping distance, sensing latency, and the intended task rather than only a static workspace diagram.

Tactile and force sensing are particularly important in manipulation because vision can anticipate contact but cannot directly measure normal force, shear, slip, local deformation, jamming, texture, or incipient breakage~\citep{tactile2025outlook}. Touch supports grasp adjustment, delicate manipulation, blind operation, and abnormal-contact detection, but tactile arrays also drift, wear, saturate, detach, and exhibit correlated errors. Visual prediction and tactile correction should therefore operate as complementary stages: exteroception evaluates the approach and surrounding hazards before contact; tactile and force sensing regulate load and detect slip or obstruction during contact; and post-contact diagnosis determines whether the object, robot, environment, and task remain in a valid state.

A significant tactile threshold exceedance or time-aligned conflict between predicted and measured contact should trigger a response appropriate to the risk and sensor health. High-risk anomalies should receive fast local authority to limit force, withdraw, or stop within a validated end-to-end latency budget. Lower-risk or ambiguous conflicts may justify slowing, re-observation, or human confirmation. High-level planning should not override local force or collision protection. Resumption should occur only after state review, fault isolation, and renewed authorization when required~\citep{tactile2025outlook,haddadin2017collisions,xspark2026architecture}.

\subsection{Computing, Communication, and Energy}
\label{subsec:computing_communication_energy}

Embodied computation spans microcontrollers, real-time processors, general-purpose CPUs, GPUs and accelerators, edge servers, and cloud services. These platforms differ in computational capacity, power consumption, timing behavior, failure modes, and the assurance evidence they can support. High-level perception, reasoning, or world modeling may tolerate variable latency or remote execution, whereas balance, braking, force regulation, collision response, and other fast protection functions require sufficiently local and predictable computation.

The architecture should distinguish hard, firm, and soft timing requirements. A missed hard deadline may immediately invalidate safety, while a firm-deadline result becomes unusable even if the miss is not itself catastrophic~\citep{limou2026embodiedaction,xspark2026architecture}. Timing failures may arise from processor overload, priority inversion~\citep{sha1990priority}, operating-system scheduling, garbage collection, cache or memory contention, thermal throttling, and long model inference. Average latency is therefore insufficient. Analysis should cover the complete sensing-to-actuation path, including tail latency, deadline misses, data freshness, and the response to stale results. A numerically correct command may still be ineffective or unsafe when executed too late.

Communication spans on-board buses, industrial networks, wireless links, edge services, and cloud connections. Delay, jitter, loss, duplication, reordering, interference, denial of service, and clock inconsistency can alter estimation, coordination, and control. Safety-relevant messages require integrity, freshness, priority, bounded retries, and explicit timeout behavior. When remote state, planning, or authority information becomes unavailable, the system should revoke capabilities whose assumptions no longer hold rather than continue following stale commands indefinitely. Local balance, load support, braking, and minimum-risk behavior must remain available during network degradation.

Computing hardware also forms part of the cybersecurity boundary. Secure boot, signed firmware, protected keys, device identity, memory protection, authenticated updates, debug-port control, and trustworthy logging reduce the chance that an attacker bypasses software-level safeguards. Physical safety and cybersecurity are inseparable at this layer because a compromised sensor processor, clock, actuator interface, or limit configuration can invalidate otherwise correct high-level reasoning.

Energy is both a resource required for useful capability and a potential hazard. Battery state, voltage sag, thermal limits, power electronics, charging behavior, and cooling determine whether the robot can compute, communicate, maintain balance, hold a load, brake, or enter a safe state. Energy management should verify that a task can be completed without consuming the reserve required for fallback or recovery. Thermal and power degradation should likewise preserve the control functions necessary for stability and minimum-risk behavior rather than indiscriminately reducing compute or torque.

\subsection{Actuators and Mechanical Embodiment}
\label{subsec:actuators_embodiment}

Actuators convert commands into force and motion and therefore form the final link between software proposals and physical consequence. Failure modes include saturation, backlash, friction changes, wear, overheating, torque-sensor drift, brake failure, hydraulic or pneumatic leakage, encoder faults, joint-limit violations, structural cracking, and cable damage. These conditions change the relationship assumed by planning and control. A trajectory that is accurate, efficient, and safe for a healthy robot may become infeasible or hazardous when available torque, braking capability, stiffness, or tracking accuracy changes.

Mechanical design can reduce the consequence of software or control error before active intervention occurs. Low inertia limits impact energy; rounded surfaces and protected pinch points reduce injury severity; and series elasticity~\citep{pratt1995sea}, variable impedance~\citep{hogan1984impedance}, compliant materials, soft structures, mechanical stops, clutches, and fail-safe brakes can limit force or preserve a stable configuration. These passive and semi-passive mechanisms remain available when perception, planning, computing, or communication fails. They strengthen the assurance case, but do not determine whether the task itself is appropriate or whether the resulting residual risk is acceptable.

Tools and payloads are part of the effective embodiment. The same collaborative arm has different capability and risk characteristics when fitted with a padded gripper, sharp tool, powered instrument, hot object, or heavy payload. Tool and payload changes affect inertia, center of mass, workspace, braking distance, balance, collision energy, sensing coverage, and control authority. They should therefore trigger configuration validation, revised operating limits, and re-evaluation of the supported deployment boundary. The same principle applies to policy transfer across robots: geometry, action scale, compliance, sensing, actuation, and timing assumptions must be re-established rather than inferred from nominal task similarity~\citep{o2024open}.

Hardware redundancy can preserve service after component failure, but also increases mass, energy use, cost, and coordination complexity. Passive fault tolerance uses robust design or redundancy to tolerate a predefined fault set without online reconfiguration. Active fault tolerance detects a fault and changes estimation, control allocation, workspace, speed, or task policy. Active schemes support broader degradation modes but depend on timely and correct diagnosis; an incorrect isolation result can itself cause harmful reconfiguration.

\subsection{Physical Human--Robot Interaction Safety}
\label{subsec:phri_safety}

Physical human--robot interaction (pHRI) demonstrates why trustworthiness must be assessed at the application level. Risk depends jointly on robot and human behavior, task geometry, contact mode, tool, payload, workspace, sensing, and control policy. A robot described as collaborative is therefore not safe in every configuration or task~\citep{iso10218}. The complete application must be designed, validated, and operated within quantitative limits~\citep{zanella2026phri}.

Protection spans several stages. Pre-contact mechanisms use separation, motion prediction, speed adaptation, virtual boundaries, approach-direction constraints, and collision avoidance. Contact-time mechanisms use force and torque limits, impedance or admittance control~\citep{hogan1984impedance}, compliance, impact detection~\citep{haddadin2017collisions}, energy limitation, and rapid withdrawal or stopping. Sustained contact requires additional analysis because repeated pressure or load may cause pain, fatigue, or injury even when a brief impact threshold is not exceeded.

No single force or energy threshold is universally safe. Consequence depends on body region, contact area, clamping, tissue stiffness, relative motion, duration, robot configuration, effective mass, and contact direction~\citep{isots15066}. A narrow or pointed contact can produce hazardous pressure at a force that would be tolerable over a padded surface, and a passive or mechanically compliant system can still store enough energy to cause harm. Force, pressure, energy, and passivity should therefore be treated as complementary quantities whose acceptable limits depend on the intended contact and application.

Context-aware limits can improve useful performance by adapting speed, force, or energy to the detected body region, contact direction, robot configuration, effective mass, and clamping condition. Such adaptation is justified only when the underlying perception, pose estimates, sensor freshness, contact classification, and stopping-distance assumptions satisfy predefined requirements. When estimates disagree, sensors degrade, latency grows, or required state becomes unobservable, the system should revert to a conservative envelope or initiate a safe transition~\citep{zanella2026phri,isots15066}. Adaptive limits should therefore be evaluated by both their performance benefit and the additional failure modes introduced by the estimation pipeline.

Human interaction also depends on legibility and predictability. People infer robot intent from motion, speed, gaze, spacing, pauses, and yielding behavior. Clear motion communication can reduce surprise and inappropriate human response, but it does not replace physical separation, force limitation, or independent stopping mechanisms. It is a complementary means of reducing exposure and supporting appropriately calibrated human trust.

\subsection{Fault Diagnosis and Fault-Tolerant Control}
\label{subsec:fault_diagnosis_control}

Fault diagnosis provides the information needed to preserve capable and safe operation after degradation. It is commonly divided into detection, isolation, and identification~\citep{haddadin2017collisions}. Detection determines whether and when a fault occurred; isolation identifies the affected component or channel; and identification estimates its type, magnitude, or progression. The response depends on all three. A system may compensate for a biased sensor, switch to another channel, redistribute joint motion after actuator degradation, restrict the task, or stop when structural integrity or control authority is uncertain~\citep{quamar2024faultdiagnosis}.

Cross-modal residuals provide one source of diagnostic evidence. For example, comparing contact predicted from vision with time-aligned tactile or force measurements can reveal calibration error, environmental change, unexpected collision, or sensor degradation. Such residuals must be interpreted using uncertainty, health state, update rate, and common dependencies. High-risk force or contact anomalies should conservatively limit motion, while lower-risk and inconclusive conflicts may justify slower operation, re-observation, or human confirmation~\citep{avizienis2004dependability,gao2015faultsurvey,quamar2024faultdiagnosis}.

Diagnostic methods provide different forms of evidence. Model-based diagnosis compares measured behavior with kinematic, dynamic, electrical, thermal, or contact predictions and uses structured residuals to support fault isolation~\citep{gao2015faultsurvey}. It is interpretable but depends on model fidelity and can be difficult for nonlinear contact or learned components. Signal-based diagnosis analyzes position, velocity, current, torque, vibration, temperature, acoustic, or force signals and can operate online, although normal changes in payload or task may resemble faults. Data-driven diagnosis captures nonlinear and multivariate patterns but is limited by rare-fault data, distribution shift, calibration, and interpretability. Hybrid approaches combine physical residuals with learned features to broaden coverage while retaining explicit physical structure.

Fault-tolerant control uses diagnosis and uncertainty to select an appropriate response. Possible actions include sensor compensation, channel switching, controller reconfiguration, actuator reallocation, reduced speed or workspace, task modification, safe unloading, or transition to a minimum-risk state. The response should account for detection delay and diagnostic uncertainty. A high-risk task should not continue unchanged merely because a classifier has not crossed a fixed threshold; progressive restriction and confidence-sensitive degradation can reduce exposure while evidence accumulates.

Digital twins can support diagnosis, recovery, and maintenance by comparing expected and observed behavior, estimating degradation, and simulating candidate reconfigurations before applying them to hardware. They can also generate controlled fault scenarios that would be dangerous or expensive to reproduce physically. Their recommendations remain bounded by synchronization, model fidelity, parameter updates, and cybersecurity. A stale or compromised twin may recommend an ineffective or unsafe recovery and should not possess independent authority over physical execution~\citep{quamar2024faultdiagnosis}.

\subsection{Hardware--Software Co-Design}
\label{subsec:hardware_software_codesign}

The hardware mechanisms discussed above contribute different but
complementary assurance functions. Table~\ref{tab:hardware_assurance_matrix}
maps the principal hardware subsystems to six system-level functions:
state observability, timing assurance, energy and force limitation,
fault detection, safe degradation, and transition to a minimum-risk
state. A checkmark identifies a primary contribution rather than an
exclusive responsibility or a complete guarantee.


\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.30}
\caption{Primary assurance functions of hardware subsystems in embodied
intelligence. Checkmarks denote principal contributions rather than
complete or independent coverage.}
\label{tab:hardware_assurance_matrix}

\begin{tabular}{
    p{0.22\textwidth}
    >{\centering\arraybackslash}p{0.105\textwidth}
    >{\centering\arraybackslash}p{0.105\textwidth}
    >{\centering\arraybackslash}p{0.105\textwidth}
    >{\centering\arraybackslash}p{0.105\textwidth}
    >{\centering\arraybackslash}p{0.105\textwidth}
    >{\centering\arraybackslash}p{0.105\textwidth}
}
\toprule

\textbf{Hardware subsystem}
&
\textbf{State observability}
&
\textbf{Timing assurance}
&
\textbf{Energy and force limits}
&
\textbf{Fault detection}
&
\textbf{Safe degradation}
&
\textbf{Minimum-risk transition}
\\

\midrule

Sensors and tactile systems
&
$\checkmark$
&
$\checkmark$
&
&
$\checkmark$
&
$\checkmark$
&
\\

Computing and communication
&
&
$\checkmark$
&
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
\\

Power and thermal systems
&
&
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
\\

Actuators and brakes
&
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
\\

Mechanical embodiment
&
&
&
$\checkmark$
&
&
$\checkmark$
&
$\checkmark$
\\

Fault diagnosis and fault-tolerant control
&
&
&
&
$\checkmark$
&
$\checkmark$
&
$\checkmark$
\\

\bottomrule
\end{tabular}
\end{table*}

Hardware assurance is strongest when capability and safety requirements are considered jointly with software design. Software should expose uncertainty, expected force, timing requirements, and recovery assumptions to hardware and low-level control functions. Sensor placement should support the states required by planning, monitoring, and diagnosis. Compute allocation should preserve critical deadlines under peak load and degraded conditions. Mechanical design should limit the consequences of unsafe software outputs, while fault diagnosis should influence capability admission and task selection rather than remain an isolated maintenance function~\citep{xspark2026architecture,industry2026systems}.

Co-design makes capability--safety trade-offs explicit. Better sensing and context estimation may permit higher speed, accuracy, and less conservative collaboration, but add cost, latency, dependencies, and new failure modes. Compliance can reduce impact while limiting precision or control bandwidth. Redundancy improves fault tolerance but adds mass and energy demand. Conservative physical limits reduce risk but may make the intended service ineffective. These trade-offs should be documented for the configured system and deployment domain, with evidence that useful task performance and acceptable physical risk remain jointly sustained.

==> sections/_bac_standards_and_research_directions.tex <==
\section{Standards, Open Challenges, and Research Directions}
\label{sec:standards_challenges}

Existing standards and assurance practices address important parts of trustworthy physical intelligence. Robot and machinery safety define hazard analysis, protective measures, integration, and validation. Physical human--robot interaction guidance translates injury and pain considerations into limits on contact, force, pressure, speed, and separation. Functional safety addresses safety-related control under random hardware and systematic faults, while intended-functionality approaches address hazards that arise without an explicit component failure. Autonomous-driving practices contribute operational design domains, scenario-based validation, fallback behavior, and staged deployment~\citep{sae2021j3016,iso21448}. AI governance, software engineering, and cybersecurity frameworks add data management, transparency, human oversight, secure development, change control, monitoring, and lifecycle responsibility~\citep{zanella2026phri,limou2026embodiedaction}.

These domains collectively support trustworthy deployment, but none alone establishes that an integrated embodied system can sustain sufficient task capability under acceptable risk. A process-compliant AI system may still generate physically infeasible actions; a validated robot controller may execute an unsafe semantic objective; and a secure communication channel does not guarantee timely or appropriate physical behavior. The purpose of this section is therefore not to propose a replacement standard, but to identify how existing domains contribute to the four planes and where additional integration, evidence, and governance are needed.

\subsection{Mapping Standardization Domains}
\label{subsec:standards_mapping}

\paragraph{Robot, machinery, and pHRI safety.}
Robot and machinery safety provide hazard analysis, risk-reduction hierarchies, guarding, emergency stopping, speed and separation monitoring, power and force limiting, integration responsibilities, and validation procedures~\citep{iso10218}. Physical human--robot interaction guidance adds body-region, contact-mode, force, pressure, speed, separation, and application-level considerations~\citep{zanella2026phri,isots15066,iso13482}. These domains offer quantitative physical constraints, but their assumptions become harder to maintain when learned systems generate tasks, tools, trajectories, and contact strategies online.

\paragraph{Functional safety and intended functionality.}
Functional safety addresses random hardware faults and systematic failures through lifecycle processes, diagnostics, redundancy, integrity requirements, and verified safe states. Intended-functionality approaches address risks caused by perception limitations, incomplete environmental models, or valid components operating under unsuitable conditions~\citep{iec61508,iso26262,iso21448}. Embodied intelligence requires both perspectives because unsafe behavior may arise from a hardware fault, software defect, insufficient task capability, distribution shift, or an invalid assumption rather than a clearly failed component.

\paragraph{AI, software, and cybersecurity governance.}
AI governance frameworks contribute data quality, risk management, transparency, human oversight, monitoring, documentation, and organizational responsibility~\citep{nist2023airmf,euaiact2024}. Software and systems engineering contribute requirements traceability, architecture, verification, configuration management, and change control. Cybersecurity contributes identity, secure communication, protected updates, vulnerability management, logging, and incident response~\citep{rose2020zerotrust}. For embodied systems, these processes must connect directly to capability authority, real-time behavior, physical constraints, and contact risk.

\paragraph{Testing and assurance.}
Scenario-based testing, simulation validation, hardware-in-the-loop testing, independent assessment, metrology, incident reporting, and assurance cases support the evidence plane~\citep{riedmaier2020scenario,kelly2004gsn,ul4600}. Learning-enabled systems add requirements for training-data provenance, model versioning, statistical uncertainty, performance drift, and repeated validation after updates. Evidence must establish not only that a safeguard exists, but that useful task performance and acceptable safety remain jointly sustained within the intended deployment boundary.

Table~\ref{tab:standards_mapping} summarizes the primary relationships between major standardization domains and the four review planes. A checkmark denotes a principal contribution rather than exclusive or complete coverage. In practice, most standards affect multiple planes indirectly through shared requirements for system integration, monitoring, validation, and lifecycle management.


\begin{table}[t]
\centering
\small
\caption{Indicative mapping of standardization domains to the four review planes.
A checkmark indicates a primary contribution.}
\label{tab:standards_mapping}
\renewcommand{\arraystretch}{1.18}
\setlength{\tabcolsep}{7pt}

\begin{tabular}{p{0.42\linewidth}cccc}
\toprule
\textbf{Standardization domain}
&
\shortstack{\textbf{Software}\\\textbf{intelligence}}
&
\shortstack{\textbf{Physical}\\\textbf{execution}}
&
\shortstack{\textbf{System}\\\textbf{governance}}
&
\shortstack{\textbf{Evidence}\\\textbf{and assurance}}
\\
\midrule

Robot and machinery safety
&  & \(\checkmark\) & \(\checkmark\) & \\

Physical human--robot interaction safety
&  & \(\checkmark\) &  & \(\checkmark\) \\

Functional safety
&  & \(\checkmark\) & \(\checkmark\) & \\

Intended functionality and ODD methods
& \(\checkmark\) &  & \(\checkmark\) & \(\checkmark\) \\

AI risk and quality management
& \(\checkmark\) &  & \(\checkmark\) & \\

Software engineering and cybersecurity
& \(\checkmark\) &  & \(\checkmark\) & \\

Testing and assurance
&  &  &  & \(\checkmark\) \\

\bottomrule
\end{tabular}
\end{table}

The mapping must be interpreted at the level of the configured system, task, embodiment, authority structure, and operating environment. Compliance with an individual process or component standard does not by itself establish end-to-end trustworthiness. Robot safety standards may constrain physical execution without validating the semantic output of a foundation model; AI governance frameworks may define lifecycle responsibilities without specifying acceptable contact limits; and cybersecurity controls may protect message integrity without guaranteeing freshness or deadline satisfaction. Trustworthy deployment therefore requires an integrated assurance argument that connects these partial contributions, identifies their assumptions, and defines the boundary within which the resulting capability--safety claim remains valid.


\subsection{Cross-Layer Technical Gaps}
\label{subsec:cross_layer_gaps}

\paragraph{Semantic constraints, uncertainty, and physical limits remain disconnected.}
Natural-language goals express context, priority, preferences, and implicit norms, whereas planners and controllers require explicit geometric, temporal, force, energy, and authority constraints. Current interfaces often discard the rationale, uncertainty, and duration of these constraints. Perception systems, world models, planners, policies, and monitors also produce incompatible confidence signals. Research is needed on machine-readable contracts that preserve task intent, safety preferences, hard constraints, uncertainty, and intervention semantics from instruction through contact.

\paragraph{Local capability and safety results do not compose automatically.}
Formal guarantees usually apply to one model, layer, or timescale. Learned components may violate their assumptions, communication delay may make state stale, and contact may change the underlying dynamics. Similarly, locally capable components can form an ineffective system when interfaces lose information or impose incompatible objectives. Compositional assurance therefore requires explicit assumptions, runtime assumption monitors, cross-layer invariants, and evidence that remains valid after integration and updates.

\paragraph{Governance must connect semantic authority to real-time protection.}
High-level governance can authorize capabilities, enforce organizational rules, and record decisions, but it cannot replace local force control, collision reflexes, braking, or hardware interlocks. Conversely, fast controllers cannot determine whether a task is semantically appropriate, authorized, or worth completing. Research should establish analyzable interfaces between task-level admission, continuous action constraints, local safety controllers, hardware protection, and human authority, including defined behavior when a governance component fails~\citep{qin2026runtimegovernance,xspark2026architecture}.

\paragraph{Long-horizon capability and recoverability are weakly integrated.}
Most methods optimize task completion or immediate constraint satisfaction. Long tasks additionally require cumulative risk management, recoverable intermediate states, checkpoints, bounded retries, diagnosis, compensating actions, and criteria for safe continuation. A system that avoids immediate violations may still enter a state from which neither the task nor a safe recovery can be completed~\citep{kim2026longhorizon}.

\paragraph{Embodiment and configuration changes invalidate inherited claims.}
Semantic task knowledge may transfer across robots, but geometry, sensors, action scaling, compliance, payload, tools, timing, braking, and contact risk remain embodiment dependent. Even small configuration changes can alter both task capability and safety margins. Generalist policies and robot fleets therefore require efficient change-impact analysis, portable constraint representations, and targeted revalidation rather than automatic inheritance of evidence.

\subsection{Evaluation and Deployment Gaps}
\label{subsec:evaluation_deployment_gaps}

Evaluation remains dominated by short tasks, average performance, and final outcomes. Benchmarks should distinguish task success, safe success, unsafe success, justified intervention, excessive conservatism, violation severity, recovery, and long-duration reliability. Procedural traces are necessary to identify whether a completed task crossed an unacceptable boundary or whether a failed task preserved a recoverable state~\citep{kim2026longhorizon,li2026safetyembodied}.

The simulation--reality gap is also an evidence-boundary problem. Visual similarity does not validate contact dynamics, force, latency, wear, rare failure, human response, or hardware degradation. Physics simulators, learned world models, and digital twins should be calibrated using task- and safety-relevant physical outcomes and used to prioritize controlled physical validation rather than replace it.

Open environments prevent exhaustive testing. Scenario coverage, statistical risk estimates, formal invariants, fault injection, operational monitoring, and incident learning must therefore be combined. Research is needed on exposure-aware metrics, principled criteria for sufficient testing, and mechanisms for detecting when environmental or system change has moved operation beyond the evidence boundary.

Human and organizational evidence remains weaker than algorithmic evidence. Takeover is often assumed rather than evaluated; maintenance, calibration, update approval, logging, incident reporting, and responsibility are frequently outside prototype studies. These processes affect whether capability and safety mechanisms remain effective after deployment and should therefore be included in operational evaluation~\citep{limou2026embodiedaction}.

\subsection{Research Agenda}
\label{subsec:future_directions}

\paragraph{1. Cross-layer capability--safety contracts.}
Develop typed and machine-readable representations of task intent, capability assumptions, safety preferences, hard constraints, uncertainty, timing, authority, and recovery. Contracts should remain monitorable across software, governance, and physical execution and support diagnosis when an assumption is violated.

\paragraph{2. Physically grounded predictive models.}
Extend world models beyond visual plausibility to represent geometry, contact, force, friction, deformability, latency, hardware health, and human behavior. Prediction uncertainty should affect planning horizon, action selection, physical validation, and runtime intervention rather than remain an auxiliary confidence output.

\paragraph{3. Governable training and execution.}
Connect constrained policy learning with capability admission, runtime monitoring, local physical protection, and human authority. Learned systems should improve the distribution of task proposals without acquiring unrestricted execution privilege. Governance mechanisms should be evaluated for latency, missed violations, unnecessary rejection, recovery failure, and their impact on useful task performance.

\paragraph{4. Recovery-centered long-horizon autonomy.}
Optimize not only immediate reward and constraint satisfaction, but also the probability of preserving safe and useful future options. Develop benchmarks for checkpoints, reversibility, cumulative risk, bounded retry, compensating action, safe failure, and restoration after semantic, communication, hardware, and contact faults.

\paragraph{5. Hardware--algorithm and cross-embodiment co-design.}
Combine tactile sensing, compliant mechanics, effective-mass estimation, energy limits, diagnostics, and learned control so that embodiment reduces the consequences of software error. Develop transferable task representations while explicitly revalidating embodiment-specific geometry, timing, force, payload, and stopping constraints.

\paragraph{6. Claim-oriented evidence infrastructure.}
Create shared scenario languages, hazard and incident taxonomies, synchronized trace formats, fault models, cross-embodiment interfaces, virtual proving grounds, and independent real-robot evaluation. Infrastructure should report coverage, exposure, blind spots, unsafe success, unnecessary intervention, and the precise claims each result supports~\citep{chen2025robotwin,chen2026robodojo}.

\paragraph{7. Continuous and human-centered assurance.}
Develop change-impact analysis for model, data, sensor, tool, policy, network, and authority updates. Connect field monitoring and incident data to regression testing without allowing uncontrolled online drift. Evaluate whether operators and affected users understand system behavior, receive usable warnings, and retain effective authority under realistic workload, latency, and organizational conditions.

\subsection{A Practical Path Forward}
\label{subsec:practical_path}

Near-term progress should prioritize bounded applications in which task requirements, embodiments, tools, physical limits, and authority can be stated explicitly. Capable learned models can operate through structured interfaces and independent local protection, with evaluation reporting both task performance and safety outcomes. Simulation and learned predictive models should expand failure exploration, followed by controlled physical validation.

Medium-term work should connect cross-layer contracts, calibrated uncertainty, recoverability, configuration-aware revalidation, and operational evidence. Standardization efforts can support this process by aligning robot safety, functional safety, AI governance, cybersecurity, and assurance practices around common system descriptions, change records, and incident traces~\citep{industry2026systems}.

Long-term open-environment operation will require continuous assurance rather than a final proof or permanent level. Systems must recognize when their assumptions and evidence no longer justify current authority, restrict operation before unacceptable risk emerges, learn from experience without losing previously validated behavior, and remain accountable to the people and organizations responsible for deployment.
